RowClone: Accelerating Data Movement and Initialization Using DRAM

In existing systems, to perform any bulk data movement operation (copy or initialization), the data has to first be read into the on-chip processor, all the way into the L1 cache, and the result of the operation must be written back to main memory. This is despite the fact that these operations do not involve any actual computation. RowClone exploits the organization and operation of commodity DRAM to perform these operations completely inside DRAM using two mechanisms. The first mechanism, Fast Parallel Mode, copies data between two rows inside the same DRAM subarray by issuing back-to-back activate commands to the source and the destination row. The second mechanism, Pipelined Serial Mode, transfers cache lines between two banks using the shared internal bus. RowClone significantly reduces the raw latency and energy consumption of bulk data copy and initialization. This reduction directly translates to improvement in performance and energy efficiency of systems running copy or initialization-intensive workloads

==> Makefile <==
DOCUMENT = paper
COPY = rowclone_toppicks
SRCS = $(wildcard *.tex)
SECTIONS = $(wildcard sections/*.tex)
PLOT_SRCS = $(wildcard plots/*.tex)
FIG_SRCS = $(wildcard figures/*.tex)
TABLES = $(wildcard tables/*.tex)
ALLTEX = $(SRCS) $(SECTIONS) $(PLOTS) $(TABLES)

FIG_PDFS = $(FIG_SRCS:%.tex=%.pdf)
PLOT_PDFS = $(PLOT_SRCS:%.tex=%.pdf)


$(COPY).pdf: $(DOCUMENT).pdf
	cp $(DOCUMENT).pdf $(COPY).pdf

$(DOCUMENT).pdf: $(ALLTEX) $(FIG_PDFS) $(PLOT_PDFS) Makefile	\
	references.bib mypaper.cls
	latexmk -pdf -bibtex paper.tex

spell-check: $(ALLTEX)
	for f in $(ALLTEX); do\
		aspell check $$f;\
	done

clean:
	latexmk -C
	rm -f *.bak


==> compile/picture.tex <==
\begin{tikzpicture}[]
  
  % Style for no padding
  \tikzset{no padding/.style={inner sep=0,outer sep=0}};
  
  \newlength{\plotheight}
  \setlength{\plotheight}{3.5cm}
  \newlength{\plotwidth}
  \setlength{\plotwidth}{7cm}
  \def \ymin {0}
  \def \ymax {80}
  \def \xmin {0}
  \def \xmax {\plotwidth}
  
  % Plot Y-label defs
  \def \plotylabel {Improvement over Baseline}
  \def \ylabelfontsize {\small}
  
  % Plot ytics defs
  \def \yticsfontsize {\scriptsize}
  \def \yticswidth {1mm}
  \tikzset{ytic/.style={anchor=east,inner xsep=0.75mm,xshift=-0mm}};
  \tikzset{y-help-line/.style={densely dotted,thin}};
  
  % Plot xtics defs
  \def \xticsfontsize {\scriptsize}
  \def \xticswidth {1mm}
  \tikzset{xtic/.style={anchor=north,inner ysep=0.75mm,yshift=-1mm}};
  
  % CStack width defs
  \newlength{\barwidth}
  \setlength{\barwidth}{0.055556\xmax}
  \newlength{\clusterwidth}
  \setlength{\clusterwidth}{3.000000\barwidth}
  \newlength{\padding}
  \setlength{\padding}{0.500000\barwidth}
  
  % Bar styles
  \tikzset{bone/.style={fill=black!5}};
  \tikzset{btwo/.style={fill=black}};
  
  % Legend defs
  \def \legendfontsize {\scriptsize}
  \tikzset{legend label/.style={anchor=base west,no padding}};
  \tikzset{legend node/.style={inner xsep=1mm,inner ysep=0.75mm,outer sep=0}};
  \def \legone {IPC Improvement}
  \def \legtwo {Energy Reduction}
  
  % Outer box
  \draw [] (0, 0) rectangle (\plotwidth, \plotheight);
  
  % Plot area node
  \node (plotarea) at (0, 0)
    [anchor=south west,no padding] {
    \begin{tikzpicture}[xscale=1,yscale=0.04375]
      \draw [] (\xmin, \ymin) -- (\xmin, \ymin);
      \draw [] (\xmax, \ymax) -- (\xmax, \ymax);
      \draw [y-help-line] (\xmin, 10.0) -- (\xmax, 10.0);
      \draw [y-help-line] (\xmin, 20.0) -- (\xmax, 20.0);
      \draw [y-help-line] (\xmin, 30.0) -- (\xmax, 30.0);
      \draw [y-help-line] (\xmin, 40.0) -- (\xmax, 40.0);
      \draw [y-help-line] (\xmin, 50.0) -- (\xmax, 50.0);
      \draw [y-help-line] (\xmin, 60.0) -- (\xmax, 60.0);
      \draw [y-help-line] (\xmin, 70.0) -- (\xmax, 70.0);
      
      % Bars
      \def \base {0}
      \draw [fill=white] (0\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 15.0 - \base);
      \draw [bone] (0\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 15.0 - \base);
      \draw [fill=white] (0\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 40.0 - \base);
      \draw [btwo] (0\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 40.0 - \base);
      \draw [fill=white] (1\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 9.0 - \base);
      \draw [bone] (1\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 9.0 - \base);
      \draw [fill=white] (1\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 32.0 - \base);
      \draw [btwo] (1\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 32.0 - \base);
      \draw [fill=white] (2\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 43.0 - \base);
      \draw [bone] (2\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 43.0 - \base);
      \draw [fill=white] (2\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 60.0 - \base);
      \draw [btwo] (2\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 60.0 - \base);
      \draw [fill=white] (3\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 4.0 - \base);
      \draw [bone] (3\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 4.0 - \base);
      \draw [fill=white] (3\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 15.0 - \base);
      \draw [btwo] (3\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 15.0 - \base);
      \draw [fill=white] (4\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 4.0 - \base);
      \draw [bone] (4\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 4.0 - \base);
      \draw [fill=white] (4\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 17.0 - \base);
      \draw [btwo] (4\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 17.0 - \base);
      \draw [fill=white] (5\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 40.0 - \base);
      \draw [bone] (5\clusterwidth + \padding + 0\barwidth, \base) rectangle ++(\barwidth, 40.0 - \base);
      \draw [fill=white] (5\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 67.0 - \base);
      \draw [btwo] (5\clusterwidth + \padding + 1\barwidth, \base) rectangle ++(\barwidth, 67.0 - \base);
    \end{tikzpicture}
  };
  \node (legend) at (plotarea.north west)
    [anchor=north west,draw,fill=white,inner xsep=1mm,inner ysep=0.75mm,outer sep=0,xshift=2mm,yshift=-2mm] {
    \begin{tikzpicture}[]
      \node (legone-node) at (0,0)
        [anchor=west,legend node] {
        \begin{tikzpicture}[]
          \node at (0,0) [legend label] {\legendfontsize{\legone\vphantom{yg}}};
          \draw [bone] (-1mm, 0mm) rectangle ++(-2mm, 2mm);
        \end{tikzpicture}
      };
      \node (legtwo-node) at (legone-node.east)
        [anchor=west,legend node] {
        \begin{tikzpicture}[]
          \node at (0,0) [legend label] {\legendfontsize{\legtwo\vphantom{yg}}};
          \draw [btwo] (-1mm, 0mm) rectangle ++(-2mm, 2mm);
        \end{tikzpicture}
      };
    \end{tikzpicture}
  };
  \node (ytics) at (0, 0)
    [anchor=south east,no padding] {
    \begin{tikzpicture}[yscale=0.04375]
      \draw [] (0, \ymin) -- (0, \ymin);
      \draw [] (0, \ymax) -- (0, \ymax);
      \draw [] (0, 10.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 10.0) [ytic] {\yticsfontsize{10\%}};
      \draw [] (0, 20.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 20.0) [ytic] {\yticsfontsize{20\%}};
      \draw [] (0, 30.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 30.0) [ytic] {\yticsfontsize{30\%}};
      \draw [] (0, 40.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 40.0) [ytic] {\yticsfontsize{40\%}};
      \draw [] (0, 50.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 50.0) [ytic] {\yticsfontsize{50\%}};
      \draw [] (0, 60.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 60.0) [ytic] {\yticsfontsize{60\%}};
      \draw [] (0, 70.0) -- ++(-\yticswidth,0);
      \node at (-\yticswidth, 70.0) [ytic] {\yticsfontsize{70\%}};
    \end{tikzpicture}
  };
  \node (xtics) at (0, 0)
    [anchor=north west,no padding] {
    \begin{tikzpicture}[xscale=1]
      \draw [] (\xmin, 0) -- (\xmin, 0);
      \draw [] (\xmax, 0) -- (\xmax, 0);
      \draw [] (0.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (0.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{bootup}};
      \draw [] (1.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (1.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{compile}};
      \draw [] (2.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (2.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{forkbench}};
      \draw [] (3.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (3.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{mcached}};
      \draw [] (4.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (4.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{mysql}};
      \draw [] (5.500000\clusterwidth, 0) -- ++(0,-\xticswidth);
      \node at (5.500000\clusterwidth, -\xticswidth) [xtic] {\xticsfontsize{shell}};
    \end{tikzpicture}
  };
  \node (ylabel) at (ytics.west)
    [anchor=south,no padding,rotate=90] {
    \begin{minipage}{\plotheight}
      \centering
      \linespread{0.85}
      \ylabelfontsize{\plotylabel}
    \end{minipage}
  };
\end{tikzpicture}


==> compile/temp.tex <==
\begin{tikzpicture}
   
  % Some default styles
  \tikzset{no padding/.style={outer sep=0pt,inner sep=0pt}};
   
  % Main plot area
  \node (plot) [] {
    \begin{tikzpicture}[yscale=0.272]
      \newlength{\plotwidth}
      \setlength{\plotwidth}{7.5cm} 
      
      \newlength{\plotheight}
      \setlength{\plotheight}{5.168cm} 
      
      \newlength{\dataheight}
      \setlength{\dataheight}{19.0cm} 
      
      \newlength{\yticswidth}
      \setlength{\yticswidth}{3pt} 
      
      % Style for help lines
      \tikzset{help line/.style={densely dotted,thin}}; 

      % plot area node
      \node (plotarea) at (0,0) [anchor=south west, minimum
        height=\plotheight, minimum width=\plotwidth] {};
       
      % Y-tics for the plot
      \node (ytics) at (0, 0) [anchor=south east, no padding] {
        \begin{tikzpicture}[yscale=0.272]
          \draw [] (0,0) -- ++(0, 0);
%          \node () [anchor=east] at (-\yticswidth-2pt, 0) {\footnotesize{0}};
%          \draw [help line] (0,0) -- ++(\plotwidth,0);
          \draw [] (0,2) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 2) {\footnotesize{2}};
 %         \draw [help line] (0,2) -- ++(\plotwidth,0);
          \draw [] (0,4) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 4) {\footnotesize{4}};
  %        \draw [help line] (0,4) -- ++(\plotwidth,0);
          \draw [] (0,6) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 6) {\footnotesize{6}};
   %       \draw [help line] (0,6) -- ++(\plotwidth,0);
          \draw [] (0,8) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 8) {\footnotesize{8}};
    %      \draw [help line] (0,8) -- ++(\plotwidth,0);
          \draw [] (0,10) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 10) {\footnotesize{10}};
     %     \draw [help line] (0,10) -- ++(\plotwidth,0);
          \draw [] (0,12) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 12) {\footnotesize{12}};
      %    \draw [help line] (0,12) -- ++(\plotwidth,0);
          \draw [] (0,14) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 14) {\footnotesize{14}};
       %   \draw [help line] (0,14) -- ++(\plotwidth,0);
          \draw [] (0,16) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 16) {\footnotesize{16}};
        %  \draw [help line] (0,16) -- ++(\plotwidth,0);
          \draw [] (0,18) -- ++(-\yticswidth, 0);
          \node () [anchor=east] at (-\yticswidth-2pt, 18) {\footnotesize{18}};
         % \draw [help line] (0,18) -- ++(\plotwidth,0);
        \end{tikzpicture}
      };

      \draw (ytics.south east) -- ++(\plotwidth,0);
       
      % Outer box
      \draw [] (0,0) rectangle (\plotwidth,\dataheight);
       
      \newlength{\rowwidth}
      \setlength{\rowwidth}{0.125\plotwidth} 
      
      \newlength{\leftpadding}
      \setlength{\leftpadding}{0.15\rowwidth} 
      
      \newlength{\barwidth}
      \setlength{\barwidth}{0.333333\rowwidth}
      \addtolength{\barwidth}{-0.666667\leftpadding} 
      
      % Bar offsets
      \newlength{\bone}
      \setlength{\bone}{\leftpadding}
      \newlength{\btwo}
      \setlength{\btwo}{\bone}
      \addtolength{\btwo}{\barwidth}
      \newlength{\bthr}
      \setlength{\bthr}{\btwo}
      \addtolength{\bthr}{\barwidth}
       
      % Row node style
      \tikzset{row/.style={no padding,minimum width=\rowwidth,anchor=south west}}; 
      
      % Bar styles
      \tikzset{bone-style/.style={pattern=north west lines}};
      \tikzset{btwo-style/.style={fill=white}};
      \tikzset{bthr-style/.style={fill=black}};
       
      % X-tics style
      \tikzset{xtic/.style={rotate=90,anchor=east}}; 
      
      % Row "twolf"
      \node (twolf) [row] 
        at (0*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 8.75);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 8.75);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 8.45);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 8.45);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 1.42);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 1.42);
        \end{tikzpicture}
      };
      \node (twolf-label) [xtic] at (twolf.south) {\footnotesize{twolf}}; 
      
      % Row "vpr"
      \node (vpr) [row] 
        at (1*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 9.76);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 9.76);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 7.01);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 7.01);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 2.22);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 2.22);
        \end{tikzpicture}
      };
      \node (vpr-label) [xtic] at (vpr.south) {\footnotesize{vpr}}; 
      
      % Row "tpcc64"
      \node (tpcc64) [row] 
        at (2*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 10.71);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 10.71);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 6.73);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 6.73);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 4.61);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 4.61);
        \end{tikzpicture}
      };
      \node (tpcc64-label) [xtic] at (tpcc64.south) {\footnotesize{tpcc64}}; 
      
      % Row "xalancbmk"
      \node (xalancbmk) [row] 
        at (3*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 15.86);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 15.86);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 14.18);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 14.18);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 8.27);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 8.27);
        \end{tikzpicture}
      };
      \node (xalancbmk-label) [xtic] at (xalancbmk.south) {\footnotesize{xalancbmk}}; 
      
      % Row "milc"
      \node (milc) [row] 
        at (4*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 16.0);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 16.0);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 15.29);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 15.29);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 1.74);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 1.74);
        \end{tikzpicture}
      };
      \node (milc-label) [xtic] at (milc.south) {\footnotesize{milc}}; 
      
      % Row "gcc"
      \node (gcc) [row] 
        at (5*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 16.23);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 16.23);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 15.08);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 15.08);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 8.02);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 8.02);
        \end{tikzpicture}
      };
      \node (gcc-label) [xtic] at (gcc.south) {\footnotesize{gcc}}; 
      
      % Row "astar"
      \node (astar) [row] 
        at (6*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 16.27);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 16.27);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 5.7);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 5.7);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 1.76);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 1.76);
        \end{tikzpicture}
      };
      \node (astar-label) [xtic] at (astar.south) {\footnotesize{astar}}; 
      
      % Row "cactusADM"
      \node (cactusADM) [row] 
        at (7*\rowwidth, 0) {
        \begin{tikzpicture}[yscale=0.272]
          \draw [fill=white] (\bone, 0) rectangle ++(\barwidth, 17.44);
          \draw [bone-style] (\bone, 0) rectangle ++(\barwidth, 17.44);
          \draw [fill=white] (\btwo, 0) rectangle ++(\barwidth, 5.23);
          \draw [btwo-style] (\btwo, 0) rectangle ++(\barwidth, 5.23);
          \draw [fill=white] (\bthr, 0) rectangle ++(\barwidth, 5.02);
          \draw [bthr-style] (\bthr, 0) rectangle ++(\barwidth, 5.02);
        \end{tikzpicture}
      };
      \node (cactusADM-label) [xtic] at (cactusADM.south) {\footnotesize{cactusADM}}; 
      
       
       
      % Legend for the plot
      \node (legend) [draw,yshift=-1mm,xshift=1mm,fill=white,inner sep=2pt,anchor=north west] 
        at (0,\dataheight) {
        \begin{tikzpicture}[]
          \node (Stream-legend) [anchor=west] {
            \begin{tikzpicture}[]
              \draw [bone-style] (0,0) rectangle (2mm, 2mm);
              \node () [no padding,anchor=west] at (3mm, 1mm) {\scriptsize{Stream}};
            \end{tikzpicture}
          };
          \node (DCP-legend) [anchor=west] 
            at (Stream-legend.east) {
            \begin{tikzpicture}[]
              \draw [btwo-style] (0,0) rectangle (2mm, 2mm);
              \node () [no padding,anchor=west] at (3mm, 1mm) {\scriptsize{DCP}};
            \end{tikzpicture}
          };
          \node (DCP-AP-legend) [anchor=west] 
            at (DCP-legend.east) {
            \begin{tikzpicture}[]
              \draw [bthr-style] (0,0) rectangle (2mm, 2mm);
              \node () [no padding,anchor=west] at (3mm, 1mm) {\scriptsize{DCP-AP}};
            \end{tikzpicture}
          };
        \end{tikzpicture}
      };
    \end{tikzpicture}
  }; 
  
   
  % Title of the plot
  \node (title) [yshift=0mm,xshift=0mm,anchor=south] 
    at (plot.north) {
    \normalsize{Prefetch Lifetime Across All Prefetches}
  }; 
  
   
  % Xlabel of the plot
  \node (xlabel) [yshift=0mm,xshift=0mm,anchor=north] 
    at (plot.south) {
    \small{Benchmarks}
  }; 
  
  % Ylabel of the plot
  \node (ylabel) [rotate=90,yshift=0mm,xshift=0mm,anchor=south] 
    at (plotarea.west) {
    \small{Prefetch Lifetime}
  };
   

  
\end{tikzpicture}



==> font.tex <==
\usepackage[T1]{fontenc}
\usepackage{pifont}

